Performance-Portable Many-Core Plasma Simulations: Porting PIConGPU to OpenPower and Beyond

With the appearance of the heterogeneous platform OpenPower,many-core accelerator devices have been coupled with Power host processors for the first time. Towards utilizing their full potential, it is worth investigating performance portable algorithms that allow to choose the best-fitting hardware for each domain-specific compute task. Suiting even the high level of parallelism on modern GPGPUs, our presented approach relies heavily on abstract meta-programming techniques, which are essential to focus on fine-grained tuning rather than code porting. With this in mind, the CUDA-based open-source plasma simulation code PIConGPU is currently being abstracted to support the heterogeneous OpenPower platform using our fast porting interface cupla, which wraps the abstract parallel C++11 kernel acceleration library Alpaka. We demonstrate how PIConGPU can benefit from the tunable kernel execution strategies of the Alpaka library, achieving portability and performance with single-source kernels on conventional CPUs, Power8 CPUs and NVIDIA GPUs.

==> content/evaluation-diff.tex <==
\section{Evaluation}
\label{evaluation}
%\begin{itemize}
%\item Question to Answer:
%  \begin{itemize}
%  \item How good can PIConAlpaka utilize the OpenPower system ?
%  \item How much elements per thread was used ?
%  \end{itemize}
%\end{itemize}

% Evaluation, System, Software ?
This section provides the evaluation of the \picongpu code\DIFaddbegin \DIFadd{~\mbox{%DIFAUXCMD
\cite{rene_widera_2016_53761} }%DIFAUXCMD
}\DIFaddend that was ported to various compute architectures
%and enhanced by the element level
(see Table~\ref{tab:hardware}).
%\item The evaluation hardware of the used compute nodes is listed in table~\ref{tab:hardware}.
%\item Table~\ref{tab:hardware} lists the hardware of all for evaluation used compute nodes.
%The code was either evaluated on all CPUs  or on one GPU device of a single compute node.
We measured the runtime and performance
%(one possible metric for a memory bound code)
of the memory-bound \picongpu Kelvin-Helmholtz instability simulation~\cite{bussmann2013radiative} for one thousand time steps in double and single precision and compared these results between the various architectures.
%DIF > 
\DIFaddbegin \DIFadd{The simulation was parameterized with the boris pusher, esirkepov current solver, yee field solver, trilinear interpolation in field gathering, electron and ion species, three dimensions, 128 cells in each dimension, sixteen particles per cell, and quadratic-spline interpolation (TSC)~\mbox{%DIFAUXCMD
\cite{hockney1988computer}}%DIFAUXCMD
. 
%DIF > 
}\DIFaddend On all CPU devices the {\openmp}~2.0 back-end was used with a block consisting of a single thread with 256 elements.
%, mapped to a hardware thread, that computes 256 cells.
On \nvidia GPUs the \cuda back-end is used with a block consisting of 256 threads with a single element.
%, mapped to a streaming multiprocessor, where each processes a single cell.
All GPU evaluations are compiled with \cuda 7.0 and all CPU evaluations with gcc 4.9.2.

\begin{table*}[!t]
  \scriptsize
  \begin{center}
    \caption{Compute nodes for evaluation (core counts in braces are HW threads).}
    %\begin{center}
    %List of utilized compute nodes for evaluation. Core counts in braces denote hardware threads.
    \begin{tabular}{ |l || c | c | c |  c | c | c |}
      \hline
      \textbf{Vendor}                       & \amd           & \intel              & \ibm                  & \nvidia\\
      \hline
      \textbf{Architecture}                 & Interlagos~\cite{amdOpteron}     & Haswell~\cite{xeonE5}             & Power8~\cite{fluhr20145}                & Kepler~\cite{k80}\\
      \hline       
      \textbf{Model}                        & Opteron 6276   & Xeon E5-2698v3      & Power8 8247-42L       & K80 GK210\\
      \hline
      \textbf{Used devices per node}        & 4              & 2                   & 2                     & 1\\
      \hline
      \textbf{Cores per device}             & 16             & 16 (32)             & 10 (80)               & 2496\\
      \hline
      %\textbf{L1 per core}                  & -              & -                   & 32 KiB                & -\\
      %\hline
      %\textbf{L2 per core}                  & -              & -                   & 512 KiB               & -\\      
      %\hline
      %\textbf{L3 per core}                  & -              & -                   & 8 MiB                 & -\\      
      %\hline      
      \textbf{Base clock frequency}         & 2.3 GHz        & 2.3  GHz            & 2.1 GHz               & 0.56  GHz\\
      \hline
      \textbf{Release date}                 & Q4/2011        & Q3/2014             & Q1/2014               & Q4/2014\\
      %\hline
      %\textbf{Peak performance(sp)}         & 4x240 GFLOPS   & 2x1177 GFLOPS       & 2x560 GFLOPS          & 2x4350 GFLOPS\\
      %\hline      
      %\textbf{Peak performance(dp)}         & 4x120 GFLOPS   & 2x588 GFLOPS        & 2x280 GFLOPS          & 2x1450 GFLOPS\\
      \hline
      \textbf{Peak performance(sp)}         & 960 GFLOPS     & 2354 GFLOPS         & 1120 GFLOPS           & 4350 GFLOPS\\
      \hline      
      \textbf{Peak performance(dp)}         & 480 GFLOPS     & 1177 GFLOPS         & 560 GFLOPS            & 1450 GFLOPS\\
      \hline
    \end{tabular}
    \label{tab:hardware}
  \end{center}
  \vspace{-3em}
\end{table*}
%\footnotetext[1]{\url{https://www.amd.com/Documents/Opteron_6000_QRG.pdf}}
%\footnotetext[2]{\url{http://ark.intel.com/de/products/81060/Intel-Xeon-Processor-E5-2698-v3-40M-Cache-2_30-GHz}}
%\footnotetext[4]{\url{http://images.nvidia.com/content/pdf/kepler/Tesla-K80-BoardSpec-07317-001-v05.pdf}}

%\begin{table*}[!htbp]
%  \scriptsize
%  \begin{center}
%    \caption{Runtime, performance and floating point (FP) efficiency of the \picongpu Kelvin-Helmholtz instability simulation for single precision (SP) and for double precision (DP)
%      on various architectures (see Table~\ref{tab:hardware}).}
%    %\begin{center}
%    \begin{tabular}{ |l || c | c | c |  c | c |}
%      \hline
%      \textbf{Architecture}                 & Opteron    & Xeon       & \power        & \multicolumn{2}{c|}{K80}\\      
%      \hline
%      \textbf{Acceleration}                 & \multicolumn{3}{c|}{\alpaka(\openmp 2)}                      & \alpaka(\cuda) & \cuda \\
%      \hline                                                                                                                           
%      \textbf{Runtime SP [s]}               & 4981           & 3074                & 4012                  & 424        & 417\\      
%      \hline                                                                                                                           
%      \textbf{Runtime DP [s]}               & 5057           & 3210                & 4318                  & 1018       & 1129\\     
%      \hline                                                                                                                           
%      %\hline                                                                                                                           
%      \textbf{Performance SP [GFLOPS]}      & 44             & 72                  & 54                    & 539        & 550\\      
%      \hline                                                                                                                           
%      \textbf{Performance DP [GFLOPS]}      & 39             & 62                  & 47                    & 199        & 179\\      
%      %\hline                                                                                                                           
%      \hline                                                                                                                           
%      \textbf{FP efficiency SP [\%]}        & 4.5            & 3                   & 4.8                   & 12.3       & 12.6\\     
%      \hline                                                                                                                           
%      \textbf{FP efficiency DP [\%]}        & 8.1            & 5.2                 & 8.3                   & 13.7       & 12.3\\
%      \hline
%    \end{tabular}
%    \label{tab:runtime}
%  \end{center}
%  \vspace{-3em}
%\end{table*}

\begin{figure}[!b]
  \centerline
      {\resizebox{\textwidth}{!}{\includegraphics{evaluation/picongpu_multiplot.pdf}}}
      \caption{\DIFdelbeginFL \DIFdelFL{Runtime }\DIFdelendFL \DIFaddbeginFL \DIFaddFL{As an example to evaluate a memory-bound PIC code, runtime }\DIFaddendFL and floating point efficiency of the \picongpu Kelvin-Helmholtz instability simulation for single precision and for double precision \DIFaddbeginFL \DIFaddFL{was measured }\DIFaddendFL on various architectures (see Table~\ref{tab:hardware})\DIFdelbeginFL \DIFdelFL{. Providing efficiency is just one possible metric to evaluate a memory-bound code}\DIFdelendFL .}
          \label{fig:multiplot}
          \vspace{-7em}
\end{figure}

% Measurement results
Figure~\ref{fig:multiplot} displays the measured runtime and efficiency of the evaluated simulation.
% GPU vs GPU
On the \nvidia K80, the differences in runtime between the native and the ported PIC code are about one percent for single precision. 
For double precision, the \alpaka based code is even faster, because \alpaka emulates double \emph{atomicAdd} using \emph{atomicCAS} instead of the slower \emph{atomicExch} used by the native \picongpu implementation.
Nevertheless, this small optimization could have been introduced easily into the native \picongpu code to achieve the same runtime results.
According to these measurements, \alpaka can keep its promise of zero-overhead abstraction on the same architecture even for rather complex applications such as \picongpu.
% CPU vs GPU
The runtime between GPU and CPU implementations differ in one order of magnitude for single precision.
However, the results need to be evaluated in relation to the theoretical peak performance of the particular architecture.
This metric is denoted as floating point efficiency in Figure~\ref{fig:multiplot}.
Regarding floating point efficiency, CPU and GPU vary by a factor of three to four on single precision and by a factor of two on double precision.
Thus, \alpaka provides not just portability between GPU and CPU, but decent performance on both.
% CPU vs CPU
All evaluated CPU architectures show similar runtime and efficiency characteristics.  
Nevertheless, the \intel architecture offers the lowest runtime and highest (theoretical) peak performance of all evaluated CPU devices.
However, there still exists some potential to increase performance, as it only provides five percent floating point efficiency on double precision.
While the IBM and AMD architectures fare slightly better with about eight percent double precision efficiency, there is still a lot of potential compared to the GPU efficiency.
By refining the \alpaka back-ends and tuning the work division, this potential can be utilized to increase the performance of the CPU architectures even more.

%\begin{figure}[tb]
%  \centerline
%      {\resizebox{0.5\textwidth}{!}{\includegraphics{evaluation/picongpu_runtime.pdf}}}
%          \caption{Runtime of \picongpu executed on \nvidia, \amd, \intel and \openpower architecture.}
%          \label{fig:ptx}
%          \vspace{-1em}
%\end{figure}




    
%\begin{itemize}
%\item \openpower system at juelich supercomputing centre
%  \begin{itemize}
%  \item 4 compute nodes.
%  \item Each compute node has two CPU sockets.
%    \begin{itemize}
%    \item Each socket is equipped with a Power8 processor (8247-42L).
%    \item Each Power8 processor has 10 cores.
%    \item Each core can handle up to 8 threads (superscalar out-of-order eight-way simultaneously multithreaded multiprocessor (SMT))
%    \item little-endian and big-endian mode
%    \item Each core has 32 KiB L1 instruction cache and 64 KiB L1 data cache
%    \item Each core has 512 KiB SRAM L2 cache
%    \item All cores share 80 MiB eDRAM L3 cache
%    \item $4 * 2 * 10 * 8 = 640$ threads total.
%    \end{itemize}
%  \item Each compute has 264 GiB main memory.
%  \item Each compute node is equiped with two \nvidia Tesla K40m
%    \begin{itemize}
%      \item Each \nvidia Tesla K40m has 12 GiB global memory.
%    \end{itemize}
%  \end{itemize}
%\end{itemize}


%\subsection{PIConAlpaka}

% How was the performance ?
%\begin{itemize}
%\item First performance measurements have shown good performance on GPU devices but bad performance on CPU devices.
%\item The bad performance is a consequence of the not implemented element level.
%\item Thus, each thread processes only a single element which results in a lot of threads oversubscribing the CPU cores.
%\item Benchmarks in \cite{zewowi2016} have shown that CPU performance can be increased when the number of threads is equal to the number of SMT-CPUs and elements are distributed equally.
%\item Because, usually processing multiple elements on the CPU increases vector unit and cache utilization.
%\end{itemize}





